DensePose 3D: Lifting Canonical Surface Maps of Articulated Objects to the Third Dimension

We tackle the problem of monocular 3D reconstruction of articulated objects like humans and animals. We contribute DensePose 3D, a method that can learn such reconstructions in a weakly supervised fashion from 2D image annotations only. This is in stark contrast with previous deformable reconstruction methods that use parametric models such as SMPL pre-trained on a large dataset of 3D object scans. Because it does not require 3D scans, DensePose 3D can be used for learning a wide range of articulated categories such as different animal species. The method learns, in an end-to-end fashion, a soft partition of a given category-specific 3D template mesh into rigid parts together with a monocular reconstruction network that predicts the part motions such that they reproject correctly onto 2D DensePose-like surface annotations of the object. The decomposition of the object into parts is regularized by expressing part assignments as a combination of the smooth eigenfunctions of the Laplace-Beltrami operator. We show significant improvements compared to state-of-the-art non-rigid structure-from-motion baselines on both synthetic and real data on categories of humans and animals.

==> qual-h36m3dpw-cvpr.tex <==
% REPLACE THIS WITH YOUR DROPBOX PATH!
\graphicspath{{/Users/romansh/Downloads/iccv/}}
% \graphicspath{{/Users/dnovotny/dropbox/kp-densification/dp3d/qualitative/v003/}}
%\graphicspath{{images/qualitative/}}
\newcommand{\cdpodir}{dpc3dpo-h36m_030_orth_c3dpo_00000_MOD.argmin_translation=False_MOD.camera_scale=True_M.l.l_canonicalization=0.1}
\newcommand{\oursdir}{dpc3dpo-h36m_048_orth_short_ablation_00006_M.l.l_canonicalization=0.1_M.l.l_part_entropy=0.001_M.l.l_local_rigidity=0.0_M.l.l_arap=0.3_MOD.num_latent_parts=10}
\newcommand{\lbocdpodir}{dpc3dpo-h36m_049_orth_lboc3dpo_00000_MOD.lbo_vertex_transform_model=translation_M.l.l_canonicalization=1.0_MOD.shape_basis_size=10}
\newcommand{\noarapdir}{dpc3dpo-h36m_048_orth_short_ablation_00010_M.l.l_canonicalization=0.1_M.l.l_part_entropy=0.001_M.l.l_local_rigidity=0.0_M.l.l_arap=0.0_MOD.num_latent_parts=10}
\newcommand{\noentrdir}{dpc3dpo-h36m_048_orth_short_ablation_00018_M.l.l_canonicalization=0.1_M.l.l_part_entropy=0.0_M.l.l_local_rigidity=0.0_M.l.l_arap=0.3_MOD.num_latent_parts=10}
\newcommand{\nocandir}{dpc3dpo-h36m_048_orth_short_ablation_00030_M.l.l_canonicalization=0.0_M.l.l_part_entropy=0.001_M.l.l_local_rigidity=0.0_M.l.l_arap=0.3_MOD.num_latent_parts=10}

\newcommand{\imh}{1.72cm}
\newcommand{\linegap}{\vspace{-0.0cm}}

% \includegraphics[trim=left bottom right top, clip]{file}
\newcommand{\methodfig}[2]{%
\includegraphics[trim=2cm 0.5cm 2cm 3.2cm, clip, height=\imh]{#1/#2.png}%
}

\newcommand{\cdpofig}[2]{%
\includegraphics[trim=1cm 0cm 1cm 1.7cm, clip, height=\imh]{#1/#2.png}%
}

\newcommand{\imfig}[2]{%
\includegraphics[height=\imh]{#1/#2_image_kp_partseg.png}%
}

% 8D274B red
% A48053 orange
% 547CA2 blue
% 8EA395 green
\newcommand{\rainbowours}{%
{\color[HTML]{8D274B}D}%
{\color[HTML]{A48053}P}%
{\color[HTML]{547CA2}3}%
{\color[HTML]{8EA395}D}%    
}

\newcommand{\methtext}[1]{\centering\scriptsize\hspace{0.01cm}\rotatebox{90}{\hspace{0.1cm}#1}\hspace{0.01cm}}

\newcommand{\comparerow}[2]{%
\begin{minipage}[c]{0.24\linewidth}\centering%
    % {\tiny\url{#1}}\\
    \imfig{#2\oursdir}{#1}\\\linegap
    % \methtext{~\textbf{\color[HTML]{960061}C3DPO \cite{Novotny2019}}}%
    % \cdpofig{#2\cdpodir}{#1_pcl_raw_solid_000_000}%
    % \cdpofig{#2\cdpodir}{#1_pcl_raw_solid_000_089}\\\linegap
    % \methtext{~~~w/o ARAP}%
    % \methodfig{\noarapdir}{#1_mesh_raw_partseg_000_000}%
    % \methodfig{\noarapdir}{#1_mesh_raw_partseg_000_089}\\\linegap
    % \methtext{~~w/o entropy}%
    % \methodfig{\noentrdir}{#1_mesh_raw_partseg_000_000}%
    % \methodfig{\noentrdir}{#1_mesh_raw_partseg_000_089}\\\linegap
    \methtext{~~~~w/o parts}%
    \methodfig{#2\lbocdpodir}{#1_mesh_raw_solid_000_000}%
    \methodfig{#2\lbocdpodir}{#1_mesh_raw_solid_000_089}\\\linegap
    \methtext{~\textbf{\rainbowours~\color[HTML]{000000}(ours)}}%
    \methodfig{#2\oursdir}{#1_mesh_raw_partseg_000_000}%
    \methodfig{#2\oursdir}{#1_mesh_raw_partseg_000_089}%
\end{minipage}}


\begin{figure*}
\comparerow{S11_Posing.58860488_000056}{}  %4
% \comparerow{S11_Greeting_2.60457274_000936}{} %
% \comparerow{S9_WalkDog.60457274_002171}{}  %3
\comparerow{S9_Photo.58860488_000671}{}%
\comparerow{outdoors_fencing_01/image_00160}{3dpw-}  %5
%\comparerow{downtown_bus_00/image_01900}{3dpw-}  %4
\comparerow{downtown_runForBus_00/image_00090}{3dpw-}\\  %
%\comparerow{downtown_arguing_00/image_00586}  %
%\comparerow{downtown_walking_00/image_00353}{3dpw-}\\  %


%\comparerow{S9_Photo.58860488_002131}\\ %4
%\comparerow{S11_Discussion_2.60457274_001436} %

% \comparerow{S9_Posing.55011271_000621}  %3
% \comparerow{S9_Purchases_1.58860488_001061}  %3
% \comparerow{S9_Smoking.58860488_000946}  % 3
% \comparerow{S9_WalkDog_1.55011271_000566}\\ %2

% \comparerow{S9_WalkDog.58860488_001296}  %3
% \comparerow{S9_WalkDog.60457274_002171}  %3
% \comparerow{S9_WalkTogether_1.58860488_000741}  % 2
% \comparerow{S11_Discussion_1.60457274_000281}\\ %4

% \comparerow{S11_Discussion_2.58860488_001166}  %3
% \comparerow{S11_Discussion_2.58860488_001626}  %4
% \comparerow{S11_Discussion_2.60457274_001436}  % 4
% \comparerow{S11_Eating_1.55011271_002091}\\ %4

% \comparerow{S11_Eating.54138969_000746}  %3
% \comparerow{S11_Greeting_2.60457274_000936}  %4
% \comparerow{S11_Phoning_2.58860488_001381}  % 3
% \comparerow{S11_Phoning_2.58860488_003406}\\ %3

% \comparerow{S11_Photo.54138969_001251}  %4
% \comparerow{S11_Posing.58860488_000056}  %4
% \comparerow{S11_Waiting_1.60457274_001841}  % 3
% \comparerow{S11_WalkDog.58860488_000716}\\ %3

% good
%\comparerow{S11_Discussion_1.60457274_000281}  %4

%\comparerow{S11_Greeting_2.60457274_000936}  %4

%\comparerow{S11_Photo_1.60457274_000291} 
%\comparerow{S9_WalkTogether.55011271_001051} 
%\comparerow{S11_WalkDog.58860488_000716}\\ % does not bend enough
%\comparerow{S11_Eating_1.55011271_002091}\\ % pose is correct but weird artifact due to bad input


%\comparerow{S9_Directions.54138969_002351}  %3
%\comparerow{S9_Photo.58860488_000671}  % 3



\caption{\textbf{Qualitative evaluation on Human 3.6M (left two images) and 3DPW (right two images)}.
From top to bottom: input image and keypoints, reconstruction with the linear model instead of parts segmentation,
and of the proposed method.%
}\label{f:h36mres}
\end{figure*}

\let\cdpodir\undefined
\let\lbocdpodir\undefined
\let\oursdir\undefined
\let\imh\undefined
\let\cdpodir\undefined
\let\oursdir\undefined
\let\imh\undefined
\let\methodfig\undefined
\let\imfig\undefined
\let\rainbowours\undefined
\let\methtext\undefined
\let\comparerow\undefined
\let\linegap\undefined
\let\cdpofig\undefined
\let\imfig\undefined
\let\rainbowours\undefined



